rTop-k: A Statistical Estimation Approach to Distributed SGD

The large communication cost for exchanging gradients between different nodes significantly limits the scalability of distributed training for large-scale learning models. Motivated by this observation, there has been significant recent interest in techniques that reduce the communication cost of distributed Stochastic Gradient Descent (SGD), with gradient sparsification techniques such as top-k and random-k shown to be particularly effective. The same observation has also motivated a separate line of work in distributed statistical estimation theory focusing on the impact of communication constraints on the estimation efficiency of different statistical models. The primary goal of this paper is to connect these two research lines and demonstrate how statistical estimation models and their analysis can lead to new insights in the design of communication-efficient training techniques. We propose a simple statistical estimation model for the stochastic gradients which captures the sparsity and skewness of their distribution. The statistically optimal communication scheme arising from the analysis of this model leads to a new sparsification technique for SGD, which concatenates random-k and top-k, considered separately in the prior literature. We show through extensive experiments on both image and language domains with CIFAR-10, ImageNet, and Penn Treebank datasets that the concatenated application of these two sparsification methods consistently and significantly outperforms either method applied alone.

==> introduction_2.tex <==
Stochastic Gradient Descent (SGD) and its variants have become the workhorse for training large machine learning models on ever growing datasets. Such large-scale training can be accelerated by partitioning datasets across multiple nodes and parallelizing the computation of the stochastic gradient; nodes can compute gradients in parallel based on their local datasets, and these local gradients can then be aggregated at a master node. However, for large models with millions of parameters, it is now well-understood that full-precision gradient aggregation is costly and the associated communication overhead can negate the savings in computation time  \cite{deepgrad}. %For example, \cite{Linetal} shows that distributing training  of AlexNet with 64 nodes leads to less than 7$\times$ speed-up compared with single-node training when nodes are connected with 1 Gbps Ethernet. However, increasing the network bandwidth to 10 Gbps in the same setting leads more than 35$\times$ speed-up in training. 
Communication is an even more significant bottleneck when training is performed over potentially slow, unreliable and expensive wireless links such as in federated learning \cite{fedreview}, where locally processing user data offers additional benefits such as privacy and personalization.  

Motivated by these observations, there has been significant recent interest in developing communication-efficient SGD methods \cite{Li, Seide, Strom, QSGD, federated0, federated1, federated2, Aji, TernGrad, signSGD, deepgrad,Wang, Wangni,vqSGD}. These works show that the communication cost of SGD can be significantly reduced by using a variety of techniques, including thresholding and sparsification of the local gradients (e.g. communicating only the top-$k$ gradients with largest magnitudes or $k$ randomly selected gradients); quantization and compression of gradients (perhaps with randomization) to a small number of bits;  and reducing the number of communication rounds by performing multiple iterations on the local dataset of each node (e.g. federated averaging). The general methodology in these works is to first propose a  technique for reducing the communication cost of SGD, and then demonstrate its effectiveness through experimental evaluations and/or prove its convergence under standard assumptions. For example, such convergence guarantees have been proven in \cite{QSGD, Qsparse-local-SGD, Stichetal, vqSGD} for various communication efficient training techniques.

In this paper, we take a different approach. We ask the following question: can we develop suitable statistical models for the stochastic gradients and use these models to inform the design of more efficient training techniques? This statistical perspective has been the focus of a recent research line in distributed estimation theory \cite{duchi,garg,braverman,raginski, yanjun,diakonikolas, archayaetal, Leightonallerton, Leightonarxiv}. Motivated by similar observations as above, these works focus on characterizing the impact of communication constraints on the estimation efficiency of common statistical models, e.g. Gaussian mean estimation and its sparse variants, and discrete distribution estimation. However, it is unclear how to leverage these results to inform new practical training methods with SGD; these works focus on a  parameter estimation framework rather the training problem, and their emphasis is on canonical statistical models such as Gaussian mean estimation, which may not accurately reflect the distribution of  the stochastic gradients.  

In this work, we connect these two research lines by casting each communication round of distributed SGD as a communication-constrained parameter estimation problem and propose a %several new
statistical model for the stochastic gradients. This model aims to capture the skewed and sparse distribution of the local gradients observed in experiments, which underlies the experimental success of existing sparsification methods such as top-$k$ and thresholding \cite{}.. These methods communicate only  a few local gradients with the largest magnitudes and can reduce the communication cost to order $k\log d$, where $d$ is the number of gradient components. They have been observed to outperform (stochastic) quantization techniques in experiments \cite{Stich}, which require at least $\sqrt{d}$ bits. 

By using the toolset of distributed estimation theory, we characterize the fundamental estimation efficiency for our proposed statistical model and the optimal communication and estimation schemes that achieve this performance. We see that the idea of randomly subsampling from the large magnitude gradients emerges naturally under the study of this statistical model.  Instead of simply choosing the top-$k$ gradients, the optimal communication scheme chooses a random $k$-subset of the gradients with large magnitudes. Even though random-$k$ and top-$k$ sparsification have both been separately considered  in the literature, their concatenated application, selecting a random subset of the top magnitude gradients, which we call rTop-$k$, is novel. It can be observed from \cite{Stich} that  rTop-$k$ readily enjoys the same convergence guarantees as top-$k$ and rand-$k$ since it is also a $k$-contraction. However, in extensive experiments on both image and language domains with CIFAR-10, ImageNet, and Penn Treebank datasets we observe that rTop-$k$ significantly outperforms either top-$k$ or random-$k$ applied separately.

The contributions of our paper can be summarized as follows:
\begin{itemize}
\item We show that each communication round of distributed SGD can be cast as a communication-constrained statistical parameter estimation problem and that the study of such problems can inform the design of communication-efficient training schemes. To the best of our knowledge, our work is the first to connect distributed stastical estimation theory with communication efficient SGD methods.
\item We propose and analyze novel statistical estimation models that capture the skew and sparse distribution of the stochastic gradients. We develop new communication and estimation schemes for these models and prove their optimality via information theoretic lower bounds.
\item We introduce a new gradient sparsification scheme, rTop-$k$,  and show that it outperforms either of its two previously known constituent schemes in extensive experiments.
\end{itemize}  

%The methods proposed in these works can be broadly grouped in three major categories:
%\begin{enumerate}
%\item Quantization of gradients, where  each node quantizes its local gradients (perhaps with randomization) to a small number of bits. The resultant bits can be potentially further compressed by using coding techniques.
%\item Sparsification of gradients, where each node chooses a subset of its local gradients and communicates them at full precision , e.g. by choosing the top-$k$ gradients with largest magnitudes, or by randomly choosing a subset of $k$ gradients.  
%\item Local training, where each node performs several SGD iterations on its local dataset before communicating a model update to the central server. 
%\end{enumerate}

%While some of these methods have been demonstrated to achieve significant reductions in communication bandwidth in various settings and experiments and have been proven to converge theoretically, it is unclear if and when such methods can come close to optimality. In particular, it is unclear if and by how much communication bandwidth can be further reduced, and whether any of these methods or their combinations  can come close to achieving optimal trade-offs between communication and accuracy for distributed training.  

%Characterizing such fundamental trade-offs has been the primary focus of another recent  research line in statistical estimation and learning theory \cite{duchi,garg,braverman,raginski, yanjun,diakonikolas, archayaetal, allerton}. These theoretical works prove tight minimax bounds for the distributed  estimation of many common statistical models under communication constraints (e.g. the Gaussian location model and its sparse variants, distribution estimation, etc.), and characterize the optimal trade-offs between estimation accuracy and communication bandwidth. Often, they also identify the statistically optimal distributed estimation schemes that achieve these optimal trade-offs. However, it is difficult to deduce concrete insights from these theoretical works for communication bandwidth reduction in practice. For example, none of the above mentioned methods for reducing the communication bandwidth of distributed SGD have been guided or justified by this theory.

%The primary goal of this paper is to connect these two research lines, one on communication-efficient training methods with SGD and the other on statistically optimal distributed estimation methods, in order to inform new practical training methods. We show that each communication round of distributed SGD can be posed as a communication-constrained distributed estimation problem. We propose a simple statistical model for the local gradients which abstracts a key characteristics observed in experiments: often  relatively few of the local gradients computed at each node have large magnitudes, while many have magnitudes close to zero. For example, this is the characteristics that seem to to underlie the success of existing sparsification methods like top-k or thresholding which only communicate a few of the local gradients with largest magnitudes. We then analyze this statistical model by using the toolset of statistical estimation. 

% in various settings and experiments by using a variety of techniques that include thresholding and sparsification of the local gradient vectors, coarse quantization and compression of each component, and reducing the number of communication rounds by performing multiple iterations on the local dataset of each node. Most of these techniques, in particular those that report high reductions in communication bandwidth (e.x. Deep Gradient Compression, which shows that $99.9\%$ of the gradient exchange in distributed SGD can be dropped), appear mostly experimental and it is not clear if and when such techniques come close to optimality. On the theoretical side, motivated by the same observations, there has been significant interest in establishing minimax rates for distributed statistical estimation and learning under communication constraints and developing optimal schemes that achieve these rates \cite{duchi,garg,braverman,raginski, yanjun,diakonikolas, archayaetal, allerton}. One of the main conclusions suggested by this research line is that to achieve the centralized single-node accuracy the number of bits per node in the distributed setting has to scale linearly in the dimension of the problem, which is equal to the number of parameters in the case of neural networks. A similar conclusion emerges from \cite{Suresh} which studies distributed mean estimation, without making any probabilistic assumptions, as well as from \cite{QSGD}, which studies   communication efficient distributed training from an optimization perspective. However, this conclusion appears inconsistent with evidence from experimental results which demonstrate orders of magnitude reduction in communication bandwidth while achieving the centralized single-node accuracy. 

% can be roughly grouped into three different categories: 1) Sparsification or thresholding methods which focus on choosing and communicating only a small number of components with large magnitude from each local gradient vector \cite{Ali, Lin}; 2) Methods for reducing the number of communication rounds by performing multiple local stochastic gradient updates before accumulating the model updates at the master node \cite{fed}; 3) Quantization or compression techniques that focus on representing each component of the gradient vector with minimal number of bits \cite{??}. However, all these ideas are experimental and lack a theoretical grounding. 

%In this paper, we propose a statistical estimation model for distributed stochastic gradient descent which takes into account some of the key statistical characteristics of stochastic gradients computed in experiments. In particular, many of the experimental results achieving large reductions in communication bandwidth exploit the fact that local gradient vectors are often sparse-like; only a small subset of the entries of each gradient vector have large magnitudes while most entries have magnitudes close to zero. We analyze a statistical model that abstracts this characteristic. We characterize the minimax rate for this model and show that the number of bits per node needed to achieve the centralized performance grows only logarithmically in the dimension of the gradient vectors and is proportional to the sparsity level. Hence, significant reductions can be achieved when the vectors are sparse. The optimal scheme is based on communicating a random subset of the large magnitude entries of each local gradient vector. We prove that this scheme achieves the optimal minimax rate by using the Fisher information framework for proving information-theoretic lower bounds for distributed estimation introduced in \cite{allerton}. We show that the new scheme can provide an order of magnitude improvement on the compression ratio of state of the art compression schemes.  For example, Deep Gradient Compression \cite{deepgrad}  achieves $99.9\%$ compression ratio for gradient exchange in distributed SGD, while we are able to achieve $99.99\%$ compression ratio without sacrificing accuracy for $n=10,\,15$ and $50$ nodes using ResNet-18 on Cifar10 and Cifar100.

%aim to study the distributed gradient aggregation problem from first principles by posing it as a distributed  statistical estimation problem under communication constraints. We characterize the communication optimal aggregation scheme that achieves the minimax risk and show that the optimal scheme comprises some of the heuristic techniques used in the prior literature. The structure of the optimal scheme also suggests a new method which can be used in conjunction with existing techniques to further reduce the total communication cost: segmentation of the gradient vector. The gradient vector can be segmented into non-overlapping segments and the gradients in each segment can be computed at a different node based on its local data points. The segments can then be concatenated at the master node to form the whole gradient vector. Segmentation can reduce the total communication cost by a factor equal to the total number of nodes, since each node computes and communicates only a segment of the gradient vector. While segmentation is reminiscent of random sampling techniques used in \cite{???}, where the gradient vector computed at each local node is randomly sub-sampled and sparsified at a certain rate, we observe that random subsampling is less-effective than segmentation as the randomness in the subsampling process leads to an imbalance between the components of the gradient vector: some gradient components are sampled and communicated by multiple nodes while some are not communicated by any. As a result the subsampling rate can not be chosen very aggresively; \cite{} use a rate which leads to each gradient component being communicated by ~20 nodes on average. Segmentation is much more aggresive as each component is computed based on data on only a single node. Indeed, it is a priori unclear whether convergence can be achieved with such an aggressive approach where the gradient vector is formed by a concatenation of different segments, each computed based on different data points. Our experimental results on CIFAR-10, ??show that this is possible without any loss in accuracy. We further provide extensive experiments which demonstrate that, when combined with existing techniques segmentation, can be used to decrease the communication cost by another two orders of magnitude by only tolerating a slight ($\leq 1\%$) decrease in overall testing accuracy.    



==> problem_formulation.tex <==
\subsection{Distributed Statistical Parameter Estimation} We begin by formulating the distributed parameter estimation problem. Our formulation follows \cite{}. Let
\begin{align*}
X_1, X_2, \cdots, X_n \overset{\text{i.i.d.}}{\sim} P_\theta, 
\end{align*}
where $\theta\in\Theta\subset \mathbb{R}^d$. We are interested in estimating the parameter $\theta$ from the samples $X_1,\dots, X_n$. Unlike the traditional statistical setting where samples $X_1,\cdots,X_n$ are available to the estimator as they are, we consider a distributed setting where each observation $X_i$ is available at a different node in a network and has to be communicated to a central node by using $k$ bits. In other words, each node has to encode its sample $X_i $ by a possibly randomized strategy $\Pi_i$ to a $k$-bit string $M_i$ independently of the other nodes and send it to the central processor. The goal of the central processor is to produce an estimate  $\hat{\theta}$ of the underlying parameter $\theta$ from the $nk$-bit transcript $M=(M_1,\ldots,M_n)$ it receives from the nodes so as to minimize the  worst case squared $\ell^2$ risk:
\begin{equation}\label{minmax}
\inf_{(\{\Pi_i\}_{i=1}^n, \hat{\theta})}\sup_{\theta\in\Theta} \mathbb{E}_{\theta}\|\hat{\theta}-\theta\|_2^2,
\end{equation}
where $\hat{\theta}(M)$ is an estimator of $\theta$ based on the transcript $M$. Note that the encoding strategies $\Pi_i$ for $i=1,\dots,n$ and the estimator $\hat{\theta}$ can be jointly designed to minimize the risk.


%In our theoretical analysis, we will be interested in two different types of protocols for communicating the samples: 
%\begin{itemize}
%\item[(1)] Independent communication protocols $\Pi \in \Pi_{\mathsf{Ind}}$: each node encodes its sample $X_i $ to a $k$-bit string $M_i$ independently of the other nodes and sends it to the central processor. The final transcript received by the cental node is $Y=(M_1,\ldots,M_n)$;
%\item[(2)]  Blackboard communication protocols $\Pi \in \Pi_{\mathsf{BB}}$ \cite{kush}: all nodes communicate via a publicly shown blackboard while the total number of bits each node can write in the final transcript $Y$ is still limited by $k$. When one node writes a message (bit) on the blackboard, all other nodes can see the content of the message and depending on the written bit another node can take the turn to write a message on the blackboard.
%\end{itemize}
%In both cases, the encoding strategies $\Pi$ can be randomized and can make use of shared (public) randomness among the nodes. Independent protocols involve no interaction between nodes while blackboard protocols are interactive, so clearly the second class  includes the first. In the sequel, we will propose independent communication protocols since these protocols are easier to implement in practice. However, our information theoretic converse bounds will be proved for the larger class of blackboard protocols $\Pi_{\mathsf{BB}}$, establishing the optimality of our proposed strategies within this larger class. 

%Under both types of protocols, the end goal is to produce an estimate  $\hat{\theta}$ of the underlying parameter $\theta$ from the $nk$-bit transcript $Y$ collected at the central node. Formally, we are interested in the following minimax problem under squared $\ell^2$ risk:
%\begin{equation}\label{minmax}
%\inf_{(\Pi,\hat{\theta})}\sup_{\theta\in\Theta} \mathbb{E}_{\theta}\|\hat{\theta}-\theta\|_2^2,
%\end{equation}
%where $\hat{\theta}(Y)$ is an estimator of $\theta$ based on the transcript $Y$. Note that with an independent communication protocol, $Y=(M_1,\ldots,M_n)$ and the messages $M_1,\ldots,M_n$ are independent.



\subsection{Gradient Aggregation in Distributed Training} We next formulate the gradient aggregation problem in distributed training with SGD as a distributed parameter estimation problem. Let $g^t=\mathbb{E}[\nabla \ell (\omega_t;(X,Y))]$ denote the gradient of the population risk in $\mathbb{R}^d$ where $\ell$ denotes the loss function, $\omega_t\in\mathbb{R}^d$ denotes the weights of the network at the current iteration $t$, and the expectation is with respect to the true distribution of the samples $(X,Y)$. Assume there are $n$ distributed nodes and each node $i$ for $i=1,\dots,n$ computes the (stochastic) gradient of the loss function with respect to  a small batch of i.i.d. samples $\{(X_{j}^{(i)}, Y_{j}^{(i)})\}_{j=1}^{B}$ available at this node,
$$
g_i^t=\frac{1}{B}\sum_{j=1}^B \nabla \ell (\omega_t;(X_{j}^{(i)},Y_{j}^{(i)})).
$$
Note that when disjoint subsets of the dataset are assigned to different nodes, $\{(X_{j}^{(i)}, Y_{j}^{(i)})\}_{j=1}^{B}$ can be modeled as independent and identically distributed for different $i$. Hence, the local gradients $g_1^t, g_2^t,\dots, g_n^t\,\in\,\mathbb{R}^d$ are generated independently from the same (unknown) distribution  and have mean equal to $g^t$, the true gradient with respect to the population risk. \footnote{The same model can be extended to the case where nodes perform multiple steps of stochastic gradient descent on their local dataset such as in federated learning \cite{federatedreview}, in which case $g_i^t$ is the resultant model update generated by node $i$.} Assume communication is bandwidth-limited and each node has $k$ bits to communicate its gradient vector $g_i^t$ to the central processor. The goal of the central node is to generate an estimate $\hat{g}^t$ of the true gradient $g^t$ under squared $\ell^2$ risk as per \eqref{minmax} from the  $nk$-bit transcript $Y$ it obtains at the end of this communication round. The $g^t$ can be regarded as the parameter of the underlying distribution that we wish to estimate. In order to complete the model description,  we need to specify the statistical model $P_\theta$, with $\theta=g^t$, according to which the samples $g_1^t, g_2^t,\dots, g_n^t$ are generated as well as the set $\Theta\subset\mathbb{R}^d$ in which the parameter lies. We do that in the following subsection.

\begin{figure}
\centering
\begin{tikzpicture}
\node at (2, 1.4) {$g^t=\mathbb{E}[\nabla \ell (\omega;(X,Y))]$}; 
\draw [->] (1.8, 1.2) -- (0.2, 0.2); 
\draw [->] (1.9, 1.2) -- (1.1, 0.2); 
\draw [->] (2.1, 1.2) -- (2.9, 0.2); 
\draw [->] (2.2, 1.2) -- (3.8, 0.2); 
\draw (0,0) circle (0.2cm); \node [below] at (0,-0.2) {$\tilde{g}_1^t$}; 
\draw (1,0) circle (0.2cm); \node [below] at (1,-0.2) {$\tilde{g}_2^t$}; 
\node at (2,0) {$\cdots$}; 
\draw (3,0) circle (0.2cm); \node [below] at (3,-0.2) {$\tilde{g}_{n-1}^{t}$}; 
\draw (4,0) circle (0.2cm); \node [below] at (4,-0.2) {$\tilde{g}_{n}^{t}$}; 
\draw [->] (0, -0.7) -- (0, -1.4); \draw [->] (1, -0.7) -- (1, -1.4); 
\draw [->] (3, -0.7) -- (3, -1.4); \draw [->] (4, -0.7) -- (4, -1.4);
\draw (-0.3,-2.5) rectangle (4.3,-1.5);  % \node at (2,-3) {transcript $Y$}; 
\node at (2,-2) {centralized processor}; 
\draw [->] (2,-2.5) -- (2, -3); \node [below] at (2,-3) {$\hat{g}^t$}; 
\node [left] at (0, -1) {$k$ bits}; \node [right] at (4,-1) {$k$ bits}; 
\end{tikzpicture}
\caption{Statistical estimation model for distributed training.}
\label{fig:fig1}
\end{figure}

\subsection{Statistical Models}

The distributed parameter estimation problem in \eqref{minmax} has been studied for specific classes of statistical models $P_\theta$ in the literature. One special case of the parameter estimation problem in \eqref{minmax} that has been of significant interest in the literature is the Gaussian case $P_\theta=\mathcal{N}(\theta,\sigma^2I_d)$ with $\Theta=\mathbb{R}^d$ which is studied in \cite{duchi,garg,braverman,yanjun}. Adopting this Gaussian model for the gradient aggregation problem would correspond to assuming that the local gradients $g_i^t$ computed at each node are i.i.d. observations of the true gradient vector $g_t$ under spherically-symmetric additive Gaussian noise. However, this Gaussian model leads to dense observation vectors $g_i^t$ which do not reflect  the observation that the distribution of the local gradients is often skewed and sparse like in experiments, with relatively few of the $d$ gradient components having large magnitudes and most components having magnitudes close to zero. 

A sparse variation of the  Gaussian mean estimation problem has been studied in \cite{garg,braverman, yanjun}, where $\Theta= \{\theta\in \mathbb{R}^d:\|\theta\|_0\le s\le d\}$. In the gradient aggregation problem, this model corresponds to assuming that the  true gradient vector $g_t$ is sparse, with only $s$ non-zero components, while the local gradients $g_i^t$ computed at each node still correspond to i.i.d. observations of the true gradient vector $g_t$ under Gaussian noise. This leads to the observation vectors $g_i^t$ to be still dense as in the original Gaussian model and qualitatively this model behaves similarly to the original Gaussian model. In particular the number of bits $k$ needed to achieve the centralized estimation performance (with no communication constraints) is not impacted by the sparsity assumption and scales linearly with the ambient dimension $d$ as in the original Gaussian model. Similarly the optimal communication scheme independently quantizes each gradient component as in the case of the dense Gaussian model.

In this work, we instead propose to focus on the following sparse Bernoulli model. Suppose each node $i$ has a sample \begin{equation}\label{eq:model} X_i \sim \prod_{j=1}^d\text{Bern}(\theta_j)\end{equation} with $$\Theta = \left\{ \theta\in[0,1]^d \, : \, \sum_{j=1}^d \theta_j \leq s \right\} \; .$$ The zero values from the Bernoulli random variables model gradient components with small magnitudes, while the one values model those components with large gradient components. The constraint $\sum_{j=1}^d \theta_j \leq s$ captures the sparsity of the stochastic gradient vectors, with most components having magnitude close to zero. While this is a highly simplified model for real stochastic gradient vectors, it can be easily extended to more accurately reflect the stochastic gradients, and doing so does not change the optimal encoding or estimation schemes. In particular, we could consider the following refinements:
\begin{itemize}
\item[(i)]{\bf Signed values:} The mean parameters $\theta_j$ could be in $[-1,1]$ so that they are positive or negative, with the $j$th component of the $X_i$ being $\mathsf{Sign}(\theta_j)\mathsf{Bern}(|\theta_j|)$.
\item[(ii)]{\bf Scaling:} The Bernoulli random variables could be scaled by any $M>0$ with the goal of estimating the scaled Bernoulli parameters $M\theta$.
\item[(iii)]{\bf Continuous Perturbations:} We could add a vector of continuous random variables $Z_i$ to each $X_i$, where each component of $Z_i$ is supported in $[-\frac{1}{2},\frac{1}{2}]$.
\end{itemize}
With none of these refinements changing the fundamental encoding and estimation schemes, we find that the simple sparse Bernoulli model captures the issues that are central to our distributed estimation problem. Note that by including just the sign and scaling changes, the resulting model makes a good representation of roughly quantized stochastic gradients such as with ternary quantization.

%\begin{thm}[Sparse Gaussian location model]\label{thm.sparse}
	%Let $P_{\theta}=\mathcal{N}(\theta,\sigma^2I_d)$ with $\Theta= \{\theta\in \mathbb{R}^d:\|\theta_0\|\le s\}$. For $k\ge \log d$ and $n\ge \frac{sd\log(d/s)}{\min(k,d)}$, we have
	%\begin{align}
	%\inf_{\left(\Pi\in\Pi_{\mathsf{BB}},\hat{\theta}\right)}\;\sup_{\theta\in\Theta} \mathbb{E}_{\theta}\|\hat{\theta}-\theta\|_2^2 =\Theta \left(\max\left(\frac{sd\sigma^2\log(d/s)}{nk}, \frac{s\sigma^2\log(d/s)}{n}\right)\right). \label{eq:sparseG}
	%\end{align}
	%\end{thm}
%
%The bound in the theorem can be achieved with a simple independent communication protocol to within a logarithmic gap. For $k\leq d$, we partition the $d$ dimensions into $d/(k/c)$ segments each of size $k/c$ for $c=\Theta(\log n)$. Each node is assigned a segment, hence each segment is assigned to $nk/dc$ different nodes. Each node $i$ only communicates the entries of its sample vector $X_i$ in its assigned segment by quantizing each entry into $c$ bits, hence using $c\times k/c$ bits in total. The central node then averages all of the quantized samples it has for each component, and sets any component to zero if it has magnitude less than a constant fraction times $\sigma/\sqrt{n}$ (see \cite{garg}).
%
%This model allows the underlying parameter $\theta$ to have $s\leq d$ non-zero components, where $s=d$ corresponds to the non-sparse case. The samples $X_i$ correspond to observations of $\theta$ under spherically-symmetric i.i.d. Gaussian noise. In the gradient aggregation problem, this would correspond to assuming that the true gradient vector $g_t$ is $s$-sparse and the local gradients $g_i^t$ computed at each node correspond to observations of $g_t$ under independent Gaussian noise. Note that under this model, even if the mean $\theta$ is assumed to be sparse, the sample vectors $X\sim\mathcal{N}(\theta,\sigma^2I_d)$ are dense since noise of constant variance is added to each entry of $\theta$. As a result, in \eqref{eq:sparseG}, the number of bits $k$ (per node) needed to achieve the centralized performance is linear in $d$ regardless of the sparsity level $s$. (The centralized performance is given by the second term in the maximization on the right side of \eqref{eq:sparseG}.) However in experiments, the stochastic gradient vectors $g_i^t$ computed at each node have been observed to be sparse-like: only a small subset of the $d$ dimensions have large magnitudes while most entries have magnitude close to zero.  Experimental results have also shown that the centralized performance can be achieved by using much fewer than $d$ bits per node. In the next section, we propose a model that better captures the statistical characteristics of the gradient vectors. 

%Nevertheless, it is worth noting that the optimal scheme for the sparse Gaussian location model suggests the idea of segmentation for communicating the sample vectors when communication budget is limited: different segments of the gradient vector can be computed by different nodes on their respective local datasets and segments can be aggregated at the central node. We experiment with this strategy in Section~\ref{sec:experiments}.

\subsection{Theoretical Results and Discussion}

%This reflects the fact that the stochastic gradient vectors, which themselves are relatively sparse, may have large entries even in locations where the true gradient vector is small. The Bernoulli model captures the fact that the entries of the stochastic gradient vectors are also sparse like, with some entries having magnitudes much larger than others. This model may also be useful for analyzing stochastic gradient vectors after they have been thresholded, where many entries are set directly to zero, or after a coarse 1-bit quantization where the entries are set directly to zero or one.

We now turn to analyzing the distributed estimation problem under this model.

\begin{thm}[sparse Bernoulli upper bound]\label{thm:sparseBernoulliUB}
For the sparse Bernoulli model \eqref{eq:model} above,
$$\inf_{(\hat\theta,\Pi_i)}\sup_{\theta\in\Theta} \mathbb{E}_\theta\|\hat\theta-\theta\|_2^2 \leq C\frac{s^2\log d}{nk}$$
for $2\log d \leq k \leq s\log d$ and some constant $C$ that is independent of $n,k,d,s$.
\end{thm}

We prove this theorem in Section~\ref{sec:SparseBUB} by describing an explicit independent encoding scheme at each node and a centralized estimator that together achieve at most this error. The scheme is built on the idea of subsampling the non-zero entries in each sample vector and communicating the locations of the subsampled components. For the gradient aggregation problem, this translates to  communicating a random subset of the large magnitude entries of the local gradient vectors. 

We also prove the following lower bound which shows that our proposed scheme is optimal within a logarithmic gap.

\begin{thm}[Sparse Bernoulli lower bound] \label{thm:sparseBernoulliLB}
For the sparse Bernoulli model \eqref{eq:model} above, if $nk \geq d\log\frac{d}{s}$ then
\begin{equation}
\sup_{\theta\in\Theta} \mathbb{E}_\theta\|\hat\theta-\theta\|_2^2 \geq c\max\left\{\frac{s^2\log \frac{d}{s}}{nk},\frac{s}{n}\right\}\label{eq:sparseBerLB}
\end{equation}
for any estimator $\hat{\theta}(M)$, communication strategies $\Pi_i$, and some constant $c$ that is independent of $n,k,d,s$.
\end{thm}

The proof of this theorem is given in the supplementary material. It builds on a geometric characterization of Fisher information from quantized samples, a framework introduced in \cite{allerton}. The two theorems together show that the number of bits $k$ (per node) needed to achieve the centralized performance is of the order of $s\log d$. (The centralized performance is given by the second term in the maximization on the right side of \eqref{eq:sparseBerLB}.) In contrast to the sparse Gaussian location model, this model suggests that the centralized performance can be achieved with much fewer than $d$ bits when the underlying vector is sparse with $s\ll d$.  

\subsection{rTop-$k$ Algorithm}
Motivated by the theoretical results for the sparse Bernoulli model, we propose the following algorithm for encoding and aggregating gradients so as to reduce the overall communication cost.
\begin{algorithm}[H]
{\bf Hyperparameters:} number of components communicated $k$, subsampling ratio $r/k$ \\
{\bf Inputs:} stochastic gradients $g_1^t,\ldots,g_n^t$ \\
{\bf Output:} an estimate $\hat g^t$ of the true gradient $g^t$ for use in gradient descent
\vspace{.1in}
\begin{algorithmic}
\STATE {$\hat g^t \gets 0$}
\FOR{$i=1,\ldots,n$} \STATE{$\hat g^t \gets \hat g^t + \mathsf{rTopEncode}(g_i^t)$} \ENDFOR
\STATE {$\hat g^t \gets \left(\frac{r}{k}\right)\cdot\hat g^t$} \\
\vspace{.1in}
\STATE $\mathsf{rTopEncode}(g_i^t):$
\STATE \hspace{.15in} $I \gets$ (indices of the $r$ largest mag. components of $g_i^t)$
\STATE \hspace{.15in} $I \gets$ (a random subset of $k$ out of the $r$ elements of $I$)
\STATE \hspace{.15in} $g \gets$ ($g_i^t$ with indices  not in $I$ set to 0)
\STATE \hspace{.15in} {\bf return} g
\vspace{.1in}
\end{algorithmic}
\caption{rTop-$k$}
\end{algorithm}
Note that using this algorithm, $k$ is the final number of components that must be communicated from each node to the centralized processor. Since the index for each component can be referred to with $\log d$ bits, and the value of each component can be encoded with a constant number of bits of precision, this is also up to logarithmic factors the number of bits needed for communication. For this reason we have used $k$ to refer to both the number of bits allowed in the distributed statistical estimation framework, and the number of gradient components that are communicated in distributed training.




==> problem_formulation_1129__Leighton_Barnes_s_conflicted_copy_2020-11-29_.tex <==
\subsection{Distributed Statistical Parameter Estimation} We begin by formulating the distributed parameter estimation problem. Let
\begin{align*}
X_1, X_2, \cdots, X_n \overset{\text{i.i.d.}}{\sim} P_\theta, 
\end{align*}
where $\theta\in\Theta\subseteq \mathbb{R}^d$. We are interested in estimating the parameter $\theta$ from the samples $X_1,\dots, X_n$. Unlike the traditional statistical setting where samples $X_1,\cdots,X_n$ are available to the estimator as they are, we consider a distributed setting where each observation $X_i$ is available at a different node in a network and has to be communicated to a master node by using $k$ bits. In other words, each node has to encode its sample $X_i $ by a possibly randomized strategy $\Pi_i$ to a $k$-bit string $M_i$ independently of the other nodes and send it to the master processor. The goal of the master node is to produce an estimate  $\hat{\theta}$ of the underlying parameter $\theta$ from the $nk$-bit transcript $M=(M_1,\ldots,M_n)$ it receives from the nodes so as to minimize the  worst case squared $\ell^2$ risk:
\begin{equation}\label{minmax}
\inf_{(\{\Pi_i\}_{i=1}^n, \hat{\theta})}\sup_{\theta\in\Theta} \mathbb{E}_{\theta}\|\hat{\theta}(M)-\theta\|_2^2,
\end{equation}
where $\hat{\theta}(M)$ is an estimator of $\theta$ based on the transcript $M$. Note that the encoding strategies $\Pi_i$ for $i=1,\dots,n$ and the estimator $\hat{\theta}$ can be jointly designed to minimize the risk.


%In our theoretical analysis, we will be interested in two different types of protocols for communicating the samples: 
%\begin{itemize}
%\item[(1)] Independent communication protocols $\Pi \in \Pi_{\mathsf{Ind}}$: each node encodes its sample $X_i $ to a $k$-bit string $M_i$ independently of the other nodes and sends it to the central processor. The final transcript received by the cental node is $Y=(M_1,\ldots,M_n)$;
%\item[(2)]  Blackboard communication protocols $\Pi \in \Pi_{\mathsf{BB}}$ \cite{kush}: all nodes communicate via a publicly shown blackboard while the total number of bits each node can write in the final transcript $Y$ is still limited by $k$. When one node writes a message (bit) on the blackboard, all other nodes can see the content of the message and depending on the written bit another node can take the turn to write a message on the blackboard.
%\end{itemize}
%In both cases, the encoding strategies $\Pi$ can be randomized and can make use of shared (public) randomness among the nodes. Independent protocols involve no interaction between nodes while blackboard protocols are interactive, so clearly the second class  includes the first. In the sequel, we will propose independent communication protocols since these protocols are easier to implement in practice. However, our information theoretic converse bounds will be proved for the larger class of blackboard protocols $\Pi_{\mathsf{BB}}$, establishing the optimality of our proposed strategies within this larger class. 

%Under both types of protocols, the end goal is to produce an estimate  $\hat{\theta}$ of the underlying parameter $\theta$ from the $nk$-bit transcript $Y$ collected at the central node. Formally, we are interested in the following minimax problem under squared $\ell^2$ risk:
%\begin{equation}\label{minmax}
%\inf_{(\Pi,\hat{\theta})}\sup_{\theta\in\Theta} \mathbb{E}_{\theta}\|\hat{\theta}-\theta\|_2^2,
%\end{equation}
%where $\hat{\theta}(Y)$ is an estimator of $\theta$ based on the transcript $Y$. Note that with an independent communication protocol, $Y=(M_1,\ldots,M_n)$ and the messages $M_1,\ldots,M_n$ are independent.



\subsection{Gradient Aggregation in Distributed Training} We next formulate the gradient aggregation problem in distributed training with SGD as a distributed parameter estimation problem. Let $g^t=\mathbb{E}[\nabla \ell (\omega_t;(X,Y))]$ denote the gradient of the population risk in $\mathbb{R}^d$ where $\ell$ denotes the loss function, $\omega_t\in\mathbb{R}^d$ denotes the weights of the network at the current iteration $t$, and the expectation is with respect to the true distribution of the samples $(X,Y)$. Assume there are $n$ distributed nodes and each node $i$ for $i=1,\dots,n$ computes the (stochastic) gradient of the loss function with respect to  a small batch of i.i.d. samples $\{(X_{j}^{(i)}, Y_{j}^{(i)})\}_{j=1}^{B}$ available at this node,
$$
g_i^t=\frac{1}{B}\sum_{j=1}^B \nabla \ell (\omega_t;(X_{j}^{(i)},Y_{j}^{(i)})).
$$
Note that when disjoint subsets of the dataset are assigned to different nodes, $\{(X_{j}^{(i)}, Y_{j}^{(i)})\}_{j=1}^{B}$ can be modeled as independent and identically distributed for different $i$. Hence, the local gradients $g_1^t, g_2^t,\dots, g_n^t\,\in\,\mathbb{R}^d$ are generated independently from the same (unknown) distribution  and have mean equal to $g^t$, the true gradient with respect to the population risk. \footnote{The same model can be extended to the case where nodes perform multiple steps of stochastic gradient descent on their local dataset such as in federated learning \cite{fedreview}, in which case $g_i^t$ is the resultant model update generated by node $i$.} To model the communication bottleneck, assume each node has $k$ bits to communicate its local gradient vector $g_i^t$ to the master node. The goal of the master node is to generate an estimate $\hat{g}^t$ of the true gradient $g^t$ under squared $\ell^2$ risk as per \eqref{minmax} from the  $nk$-bit transcript $M$ it obtains at the end of this communication round. The $g^t$ can be regarded as the parameter of the underlying distribution that we wish to estimate. In order to complete the model description,  we need to specify the statistical model $P_\theta$, with $\theta=g^t$, according to which the samples $g_1^t, g_2^t,\dots, g_n^t$ are generated and the set $\Theta\subseteq\mathbb{R}^d$ in which the parameter lies.

\begin{figure}
\centering
\begin{tikzpicture}
\node at (2, 1.4) {$g^t=\mathbb{E}[\nabla \ell (\omega;(X,Y))]$}; 
\draw [->] (1.8, 1.2) -- (0.2, 0.2); 
\draw [->] (1.9, 1.2) -- (1.1, 0.2); 
\draw [->] (2.1, 1.2) -- (2.9, 0.2); 
\draw [->] (2.2, 1.2) -- (3.8, 0.2); 
\draw (0,0) circle (0.2cm); \node [below] at (0,-0.2) {$\tilde{g}_1^t$}; 
\draw (1,0) circle (0.2cm); \node [below] at (1,-0.2) {$\tilde{g}_2^t$}; 
\node at (2,0) {$\cdots$}; 
\draw (3,0) circle (0.2cm); \node [below] at (3,-0.2) {$\tilde{g}_{n-1}^{t}$}; 
\draw (4,0) circle (0.2cm); \node [below] at (4,-0.2) {$\tilde{g}_{n}^{t}$}; 
\draw [->] (0, -0.7) -- (0, -1.4); \draw [->] (1, -0.7) -- (1, -1.4); 
\draw [->] (3, -0.7) -- (3, -1.4); \draw [->] (4, -0.7) -- (4, -1.4);
\draw (-0.3,-2.5) rectangle (4.3,-1.5);  % \node at (2,-3) {transcript $Y$}; 
\node at (2,-2) {centralized processor}; 
\draw [->] (4.3,-2) -- (5, -2); \node [right] at (5,-2) {$\hat{g}^t$}; 
%\draw [->] (2,-2.5) -- (2, -3); \node [below] at (2,-3) {$\hat{g}^t$}; 
\node [left] at (0, -1) {$k$ bits}; \node [right] at (4,-1) {$k$ bits}; 
\end{tikzpicture} 
\caption{Statistical estimation model for distributed training.}
\label{fig:fig1}
\end{figure} 

\subsection{Statistical Models}

The distributed parameter estimation problem in \eqref{minmax} has been studied for specific classes of statistical models $P_\theta$ in the literature. One canonical model that has been of significant interest in the literature is the Gaussian location model $P_\theta=\mathcal{N}(\theta,\sigma^2I_d)$ with $\Theta=\mathbb{R}^d$ which is studied in \cite{duchi,garg,braverman,yanjun}. Adopting this Gaussian model for the gradient aggregation problem would correspond to modeling the local gradients $g_i^t$ computed at each node as i.i.d. observations of the true gradient vector $g_t$ under spherically-symmetric additive Gaussian noise. However, this leads to dense observation vectors $g_i^t$, while the distribution of the local gradients is often skewed and sparse like in experiments, i.e. often relatively few entries of $g_i^t$ have large magnitudes and many entries have magnitudes close to zero. 

A sparse variation of the Gaussian mean estimation problem has been studied in \cite{garg,braverman, yanjun}, where $\Theta= \{\theta\in \mathbb{R}^d:\|\theta\|_0\le s\le d\}$. Adopting this statistical model for the gradient aggregation problem would correspond to modeling the true gradient vector $g_t$ as sparse, with only $s$ non-zero components, while the local gradients $g_i^t$ computed at each node would still correspond to i.i.d. observations of the true gradient vector $g_t$ under additive Gaussian noise. Even though the true gradient vector $g_t$ is assumed to be sparse, qualitatively this model behaves similarly to the original Gaussian model. In particular the number of bits $k$ needed to achieve the centralized estimation performance (with no communication constraints) scales linearly with the ambient dimension $d$ as in the original Gaussian model, i.e. it is not impacted by the sparsity $s$. Similarly the optimal communication scheme independently quantizes each gradient component as in the case of the dense Gaussian model.

In this work, we instead propose to focus on the following sparse Bernoulli model. Suppose each node $i$ has a sample \begin{equation}\label{eq:model} X_i \sim \prod_{j=1}^d\text{Bern}(\theta_j)\end{equation} with $$\Theta = \left\{ \theta\in[0,1]^d \, : \, \sum_{j=1}^d \theta_j \leq s \right\} \; .$$ This model imposes a soft sparsity constraint on the parameter vector $\theta$; when $s\ll d$ not all entries of $\theta$ can be large, i.e. close to `1'. The observation vectors $X_i$ are highly skewed with entries either equal to `1' or `0'. Note also that the parameter vector $\theta$ corresponds to the mean of the observation vectors $X_i$. We adopt this model for the gradient aggregation problem with the understanding that $\theta=|g_t|$ and the `0' values from the Bernoulli random variables model entries of $g_i^t$ with small magnitudes, while the `1' values model entries with large magnitudes. Note that a large value for a given component of $\theta=|g_t|$ makes it more likely to observe `1', i.e. a large magnitude entry in the corresponding location of the stochastic gradient vectors $g_i^t$ for $i=1,\dots,n$. However, it does not exclude the possibility of observing a `0' i.e. a small magnitude entry, in the same location.

While this is a highly simplified model for real stochastic gradient vectors, it allows us to focus our attention on the impact of a highly skewed distribution for the magnitudes of the gradients. This model and our main results in the next section can be easily extended to more accurately reflect the distribution of the stochastic gradients, and doing so does not change the optimal encoding or estimation schemes. In particular, we could consider the following refinements:
\begin{itemize}
\item[(i)]{\bf Signed values:} The mean parameters $\theta_j$ could be in $[-1,1]$ subject to $\sum_{j=1}^d |\theta_j| \leq s$, so that  $\theta_j$'s can be positive or negative, with the $j$th component of the $X_i$ now being $\mathsf{Sign}(\theta_j)\mathsf{Bern}(|\theta_j|)$.
\item[(ii)]{\bf Scaling:} The Bernoulli random variables could be scaled by any $M>0$ with the goal of estimating the scaled Bernoulli parameters $M\theta$.
\item[(iii)]{\bf Continuous Perturbations:} We could add a vector of continuous independent zero-mean random variables $Z_i$ to each $X_i$,  where $X_i$ is distributed according to \eqref{eq:model} and each component of $Z_i$ is supported in $[-\frac{1}{2},\frac{1}{2}]$. As a result, each component of the resultant $Y_i=Z_i+X_i$ will now take continuous values.
\end{itemize}
With none of these refinements changing the fundamental encoding and estimation schemes, we find that the simple sparse Bernoulli model captures the issues that are central to our distributed estimation problem. Note that by including just the sign and scaling changes, the resulting model also makes a good representation of coarsely quantized stochastic gradients such as with ternary quantization.

%\begin{thm}[Sparse Gaussian location model]\label{thm.sparse}
	%Let $P_{\theta}=\mathcal{N}(\theta,\sigma^2I_d)$ with $\Theta= \{\theta\in \mathbb{R}^d:\|\theta_0\|\le s\}$. For $k\ge \log d$ and $n\ge \frac{sd\log(d/s)}{\min(k,d)}$, we have
	%\begin{align}
	%\inf_{\left(\Pi\in\Pi_{\mathsf{BB}},\hat{\theta}\right)}\;\sup_{\theta\in\Theta} \mathbb{E}_{\theta}\|\hat{\theta}-\theta\|_2^2 =\Theta \left(\max\left(\frac{sd\sigma^2\log(d/s)}{nk}, \frac{s\sigma^2\log(d/s)}{n}\right)\right). \label{eq:sparseG}
	%\end{align}
	%\end{thm}
%
%The bound in the theorem can be achieved with a simple independent communication protocol to within a logarithmic gap. For $k\leq d$, we partition the $d$ dimensions into $d/(k/c)$ segments each of size $k/c$ for $c=\Theta(\log n)$. Each node is assigned a segment, hence each segment is assigned to $nk/dc$ different nodes. Each node $i$ only communicates the entries of its sample vector $X_i$ in its assigned segment by quantizing each entry into $c$ bits, hence using $c\times k/c$ bits in total. The central node then averages all of the quantized samples it has for each component, and sets any component to zero if it has magnitude less than a constant fraction times $\sigma/\sqrt{n}$ (see \cite{garg}).
%
%This model allows the underlying parameter $\theta$ to have $s\leq d$ non-zero components, where $s=d$ corresponds to the non-sparse case. The samples $X_i$ correspond to observations of $\theta$ under spherically-symmetric i.i.d. Gaussian noise. In the gradient aggregation problem, this would correspond to assuming that the true gradient vector $g_t$ is $s$-sparse and the local gradients $g_i^t$ computed at each node correspond to observations of $g_t$ under independent Gaussian noise. Note that under this model, even if the mean $\theta$ is assumed to be sparse, the sample vectors $X\sim\mathcal{N}(\theta,\sigma^2I_d)$ are dense since noise of constant variance is added to each entry of $\theta$. As a result, in \eqref{eq:sparseG}, the number of bits $k$ (per node) needed to achieve the centralized performance is linear in $d$ regardless of the sparsity level $s$. (The centralized performance is given by the second term in the maximization on the right side of \eqref{eq:sparseG}.) However in experiments, the stochastic gradient vectors $g_i^t$ computed at each node have been observed to be sparse-like: only a small subset of the $d$ dimensions have large magnitudes while most entries have magnitude close to zero.  Experimental results have also shown that the centralized performance can be achieved by using much fewer than $d$ bits per node. In the next section, we propose a model that better captures the statistical characteristics of the gradient vectors. 

%Nevertheless, it is worth noting that the optimal scheme for the sparse Gaussian location model suggests the idea of segmentation for communicating the sample vectors when communication budget is limited: different segments of the gradient vector can be computed by different nodes on their respective local datasets and segments can be aggregated at the central node. We experiment with this strategy in Section~\ref{sec:experiments}.

\subsection{Theoretical Results and Discussion}

%This reflects the fact that the stochastic gradient vectors, which themselves are relatively sparse, may have large entries even in locations where the true gradient vector is small. The Bernoulli model captures the fact that the entries of the stochastic gradient vectors are also sparse like, with some entries having magnitudes much larger than others. This model may also be useful for analyzing stochastic gradient vectors after they have been thresholded, where many entries are set directly to zero, or after a coarse 1-bit quantization where the entries are set directly to zero or one.

We now turn to analyzing the distributed estimation problem under this model.

\begin{thm}[sparse Bernoulli upper bound]\label{thm:sparseBernoulliUB}
For the sparse Bernoulli model \eqref{eq:model} above,
$$\inf_{(\hat\theta,\Pi_i)}\sup_{\theta\in\Theta} \mathbb{E}_\theta\|\hat\theta-\theta\|_2^2 \leq C\frac{s^2\log d}{nk}$$
for $2\log d \leq k \leq s\log d$ and some constant $C$ that is independent of $n,k,d,s$.
\end{thm}

We prove this theorem in Section~\ref{sec:SparseBUB} by describing an explicit independent encoding scheme at each node and a centralized estimator that together achieve at most this error. The scheme is built on the idea of subsampling the non-zero entries in each sample vector and communicating the locations of the subsampled components. With signed values as in (i) above, the scheme is modified to communicate also the sign of each subsampled component. Since this requires only a single bit for each subsampled component it does change the scalings in Theorem~\ref{thm:sparseBernoulliUB}. Similarly, the constant scaling in (ii) also does not impact the scheme and the result of Theorem~\ref{thm:sparseBernoulliUB}. When continuous perturbations are present as in (iii), the scheme is modified to include a pre-processing step where $Y_i$ is quantized to `0' if $|Y_i|\leq 1/2$, and quantized to `1' if $|Y_i|>1/2$. This converts the observations to the original Bernoulli model, on which we apply the idea of random subsampling. This recovers the result in Theorem~\ref{thm:sparseBernoulliUB}. Note that this strategy is different than simply communicating the components of $Y_i$ with largest magnitude or the indexes of these large magnitude components.

We also prove the following lower bound which shows that our proposed scheme is order optimal up to logarithmic factors.

\begin{thm}[Sparse Bernoulli lower bound] \label{thm:sparseBernoulliLB}
For the sparse Bernoulli model \eqref{eq:model} above, if $nk \geq d\log\frac{d}{s}$ and $s\leq\frac{d}{2}$ then
\begin{equation}
\sup_{\theta\in\Theta} \mathbb{E}_\theta\|\hat\theta-\theta\|_2^2 \geq c\max\left\{\frac{s^2\log \frac{d}{s}}{nk},\frac{s}{n}\right\}\label{eq:sparseBerLB}
\end{equation}
for any estimator $\hat{\theta}(M)$, communication strategies $\Pi_i$, and some constant $c$ that is independent of $n,k,d,s$.
\end{thm} 
The proof is given in Section~\ref{sec:pf2}. It builds on a geometric characterization of Fisher information from quantized samples, a framework introduced in \cite{allerton}. The same lower bound applies trivially to extensions (i) and (ii) above, while the extension to (iii) follows simply from the data processing inequality for Fisher information. The two theorems together show that the number of bits $k$ (per node) needed to achieve the centralized performance under the sparse Bernoulli model is of the order of $s\log d$. (The centralized performance is given by the second term in the maximization on the right side of \eqref{eq:sparseBerLB}.) This model is interesting from a statistical estimation perspective; in contrast to the sparse Gaussian location model, this model suggests that the centralized performance can be achieved with much fewer than $d$ bits when the underlying vector is sparse with $s\ll d$.  

\subsection{rTop-$k$ Algorithm}
\label{sec:rtopk}
The main algorithmic idea that emerges from the theoretical analysis of the sparse Bernoulli model is to communicate a random subset of the large magnitude entries of the local gradient vectors. Motivated by this observation, we propose a new sparsification operator rTop-k for sparsifying the local gradient vectors, so as to reduce the overall communication cost of distributed SGD. This new sparsification operator can be viewed as a concatenation of top-$r$ and random-$k$ sparsification operators from the prior literature.

\begin{defn}[top-$r$ sparsification \cite{Aji,deepgrad,Stichetal,Qsparse-local-SGD}]
For a parameter $1\leq r\leq d$, the operator top-$r$: $\mathbb{R}^d\rightarrow\mathbb{R}^d$ is defined for $\omega \in\mathbb{R}^d$ as
$$
\left(\text{top-}r(\omega)\right)_i :=\begin{cases} (\omega)_{\pi(i)}, & \; \text{if} \; i\leq r \\ 0 & \; \text{otherwise ,} \end{cases}
$$
where $\pi$ is a permutation of $[d]:=\{1,\dots,d\}$ such that $(|\omega|)_{\pi(i)}\geq(|\omega|)_{\pi(i+1)}$ for $i=1,\dots, d-1$.
\end{defn}

\begin{defn}[random-$k$ sparsification \cite{federated2, Stichetal,Qsparse-local-SGD}]
For a parameter $1\leq k\leq d$, let $\mathcal{W}_k$ denote the set of all $k$ element subsets of $[d]$ and $w$ be uniformly at random chosen element of $\mathcal{W}_k$. The operator random-$k$: $\mathbb{R}^d\rightarrow\mathbb{R}^d$ is defined for $\omega \in\mathbb{R}^d$ as
$$
\left(\text{random-}k(\omega)\right)_i :=\begin{cases} (\omega)_{i}, & \; \text{if} \; i\in w \\ 0 & \; \text{otherwise.} \end{cases}
$$
\end{defn}

\begin{defn}[rTop-$k$ sparsification]
For two parameters $1\leq k\leq r\leq d$, the operator rTop-$k$: $\mathbb{R}^d\rightarrow\mathbb{R}^d$ is defined for $\omega \in\mathbb{R}^d$ as
$$
\text{rTop-}k (\omega)\,=\,\text{random-}k(\text{top-}r(\omega)).
$$
\end{defn}


%
%\begin{algorithm}[h]
%{\bf Hyperparameters:} number of components communicated $k$, subsampling ratio $r/k$ \\
%{\bf Inputs:} stochastic gradients $g_1^t,\ldots,g_n^t$ \\
%{\bf Output:} an estimate $\hat g^t$ of the true gradient $g^t$ \\
%\vspace{-.2in}
%\begin{algorithmic}
%\State {$\hat g^t \gets 0$}
%\For{$i=1,\ldots,n$} \State{$\hat g^t \gets \hat g^t + \mathsf{rTopEncode}(g_i^t)$} \EndFor
%\State {$\hat g^t \gets \left(\frac{r}{nk}\right)\cdot\hat g^t$} \\
%\State $\mathsf{rTopEncode}(g_i^t):$
%\State \hspace{.15in} $I \gets$ (indices of the $r$ largest mag. components of $g_i^t)$
%\State \hspace{.15in} $I \gets$ (a random subset of $k$ out of the $r$ elements of $I$)
%\State \hspace{.15in} $g \gets$ ($g_i^t$ with indices  not in $I$ set to 0)
%\State \hspace{.15in} {\bf return} g
%%\vspace{.1in}
%\end{algorithmic}
%\caption{rTop-$k$}
%\label{algorithm_rtopk}
%\end{algorithm}

The rTop-$k$ sparsification operator first chooses the $r$ entries with largest magnitudes of a vector $\omega\in\mathbb{R}^d$ and then communicates $k$ randomly chosen gradients among these $r$ entries. Note that while both top-$r$ and random-$k$ strategies have been studied extensively in the prior literature, their concatenated application has not been investigated in prior works. As we demonstrate in the next section, rTop-$k$ consistently outperforms either top-$r$ or random-$k$ applied alone in experiments. Intuitively, top-$r$ sparsification allows to focus only on the most significant entries of the gradient vector and random-$k$ sparsification allows to reduce the bias introduced by top-$r$ sparsification, hence concatenation combines the best of the two approaches. 

Note that using this algorithm, $k$ is the final number of components that must be communicated from each node to the centralized processor. Since the index for each component can be referred to with $\log d$ bits, and the value of each component can be encoded with a constant number of bits of precision, this is also up to logarithmic factors the number of bits needed for communication. For this reason we have used $k$ to refer to both the number of bits allowed in the distributed statistical estimation framework, and the number of gradient components that are communicated in distributed training.

%In Algorithm \ref{algorithm_rtopk_memory}, we show how the rTop-$k$ procedure can be used in distributed SGD with gradient accumulation \cite{deepgrad}. This is the algorithm we use for the simulations in the subsequent section. Distributed SGD with gradient accumulation and compression of the gradients via a ``$k$-contraction'' or ``compression operator'' has been analyzed in \cite{Stichetal} and \cite{Qsparse-local-SGD}, respectively. In these works they show for such operators (Definition 2.1 in \cite{Stichetal} and Definition 3 in \cite{Qsparse-local-SGD}), the SGD converges in the strongly convex \cite{Stichetal} and smooth but non-convex \cite{Qsparse-local-SGD} cases, and they also give upper bounds on the convergence rate. It is straightforward to show that rTop-$k$ satisfies these contraction/compression properties, and so the convergence of Algorithm \ref{algorithm_rtopk_memory} is guaranteed in these same cases by these same results. These results differ somewhat from the standard proofs of SGD convergence in that the gradient estimates can be unbiased, as is the case for rTop-$k$, however this does not affect the convergence of the algorithm.

The convergence of distributed SGD with sparsification operators top-$r$ and random-$k$ has been analyzed in the prior literature. Together with some form of error compensation, these methods have been shown to converge as fast as vanilla SGD in \cite{Qsparse-local-SGD, Stichetal, Stichnew}. Therefore, when applying rTop-$k$ sparsification to distributed SGD we also employ error compensation.  The algorithm we use for our simulations in the subsequent section is given in Algorithm \ref{algorithm_rtopk_memory}. In the next subsection, we prove that Algorithm \ref{algorithm_rtopk_memory} converges as  vanilla SGD for smooth but non-convex functions by building on the results of  
\cite{Qsparse-local-SGD}. We note that this convergence result differs somewhat from the standard proofs of SGD convergence in that the gradient estimates can be unbiased, as is the case for rTop-$k$, however this does not affect the convergence of the algorithm when error compensation is employed.


\begin{algorithm}[!h]
{\bf Hyperparameters:} number of components communicated $k$, subsampling ratio $r/k$, learning rate $\eta$, minibatch size $B$ \\
%{\bf Inputs:} stochastic gradients $g_1^t,\ldots,g_n^t$ \\
{\bf Inputs:} training data $(X^{(i)}, Y^{(i)})$ \\
%{\bf Output:} an estimate $\hat g^t$ of the true gradient $g^t$ \\
{\bf Output:} weights $\omega^T$ \\
\vspace{-.2in}
\begin{algorithmic}
\State{Broadcast randomly initialized weights, $\omega^0$, to all nodes.}
\State{$m_i^0 \gets 0$}
\For{$t=0,\ldots,T-1$} \\
\hspace{.15in} \underline{\textbf{On Nodes:}}
%\State{$\hat g^t \gets 0$}
\For{$i=1,\ldots,n$} 
\State{receive $\omega^{t}$ from the centralized processor.}
\State{$g_i^t \gets \frac{1}{B} \sum_{j=1}^B\nabla \ell (\omega_t;(X_j^{(i)}, Y_j^{(i)}))$}
\State{$g_i^t \gets g_i^t+ m_i^t$}
\State{$\hat g_i^t \gets  \mathsf{rTop}-$k$(g_i^t)$}
\State{$m_i^{t+1} \gets$ $g_i^t-\hat g_i^t$}
\State{send $\hat g_i^t$ to the centralized processor.} \EndFor \\
\hspace{.15in} \underline{\textbf{On Centralized Processor:}}
\State{receive $\hat g_i^t$s from $n$ nodes.}
\State{$\hat g^t \gets \left(\frac{r}{nk}\right)\cdot\sum_{i=1}^n \hat g_i^t$}  
\State {$\omega^{t+1} \gets \omega^{t} + \eta \cdot \hat g^t$} 
\State{broadcast $\omega^{t+1}$ to all nodes.}
\EndFor \\
\State $\mathsf{rTop}-k\,(g_i^t):$
%\State \hspace{.15in} $g_i^t \gets g_i^t+ m_i^t$
\State \hspace{.15in} $I \gets$ (indices of the $r$ largest mag. components of $g_i^t)$
\State \hspace{.15in} $I \gets$ (a random subset of $k$ out of the $r$ elements of $I$)
\State \hspace{.15in} $\hat g_i^t \gets$ ($g_i^t$ with indices  not in $I$ set to 0)
%\State \hspace{.15in} $m_i^{t+1} \gets$ $g_i^t-\hat g_i^t$
\State \hspace{.15in} {\bf return} $\hat g_i^t$ %, $m_i^{t+1}$
%\vspace{.1in}
\end{algorithmic}
\caption{SGD with rTop-$k$ and Gradient Accumulation}
\label{algorithm_rtopk_memory}
\end{algorithm}



==> problem_formulation_2.tex <==
\subsection{Distributed Statistical Parameter Estimation} We begin by formulating the distributed parameter estimation problem. Let
\begin{align*}
X_1, X_2, \cdots, X_n \overset{\text{i.i.d.}}{\sim} P_\theta, 
\end{align*}
where $\theta\in\Theta\subseteq \mathbb{R}^d$. We are interested in estimating the parameter $\theta$ from the samples $X_1,\dots, X_n$. Unlike the traditional statistical setting where samples $X_1,\cdots,X_n$ are available to the estimator as they are, we consider a distributed setting where each observation $X_i$ is available at a different node in a network and has to be communicated to a master node by using $k$ bits. In other words, each node has to encode its sample $X_i $ by a possibly randomized strategy $\Pi_i$ to a $k$-bit string $M_i$ independently of the other nodes and send it to the master processor. The goal of the master node is to produce an estimate  $\hat{\theta}$ of the underlying parameter $\theta$ from the $nk$-bit transcript $M=(M_1,\ldots,M_n)$ it receives from the nodes so as to minimize the  worst case squared $\ell^2$ risk:
\begin{equation}\label{minmax}
\inf_{(\{\Pi_i\}_{i=1}^n, \hat{\theta})}\sup_{\theta\in\Theta} \mathbb{E}_{\theta}\|\hat{\theta}(M)-\theta\|_2^2,
\end{equation}
where $\hat{\theta}(M)$ is an estimator of $\theta$ based on the transcript $M$. Note that the encoding strategies $\Pi_i$ for $i=1,\dots,n$ and the estimator $\hat{\theta}$ can be jointly designed to minimize the risk.


%In our theoretical analysis, we will be interested in two different types of protocols for communicating the samples: 
%\begin{itemize}
%\item[(1)] Independent communication protocols $\Pi \in \Pi_{\mathsf{Ind}}$: each node encodes its sample $X_i $ to a $k$-bit string $M_i$ independently of the other nodes and sends it to the central processor. The final transcript received by the cental node is $Y=(M_1,\ldots,M_n)$;
%\item[(2)]  Blackboard communication protocols $\Pi \in \Pi_{\mathsf{BB}}$ \cite{kush}: all nodes communicate via a publicly shown blackboard while the total number of bits each node can write in the final transcript $Y$ is still limited by $k$. When one node writes a message (bit) on the blackboard, all other nodes can see the content of the message and depending on the written bit another node can take the turn to write a message on the blackboard.
%\end{itemize}
%In both cases, the encoding strategies $\Pi$ can be randomized and can make use of shared (public) randomness among the nodes. Independent protocols involve no interaction between nodes while blackboard protocols are interactive, so clearly the second class  includes the first. In the sequel, we will propose independent communication protocols since these protocols are easier to implement in practice. However, our information theoretic converse bounds will be proved for the larger class of blackboard protocols $\Pi_{\mathsf{BB}}$, establishing the optimality of our proposed strategies within this larger class. 

%Under both types of protocols, the end goal is to produce an estimate  $\hat{\theta}$ of the underlying parameter $\theta$ from the $nk$-bit transcript $Y$ collected at the central node. Formally, we are interested in the following minimax problem under squared $\ell^2$ risk:
%\begin{equation}\label{minmax}
%\inf_{(\Pi,\hat{\theta})}\sup_{\theta\in\Theta} \mathbb{E}_{\theta}\|\hat{\theta}-\theta\|_2^2,
%\end{equation}
%where $\hat{\theta}(Y)$ is an estimator of $\theta$ based on the transcript $Y$. Note that with an independent communication protocol, $Y=(M_1,\ldots,M_n)$ and the messages $M_1,\ldots,M_n$ are independent.



\subsection{Gradient Aggregation in Distributed Training} We next formulate the gradient aggregation problem in distributed training with SGD as a distributed parameter estimation problem. Let $g^t=\mathbb{E}[\nabla \ell (\omega_t;(X,Y))]$ denote the gradient of the population risk in $\mathbb{R}^d$ where $\ell$ denotes the loss function, $\omega_t\in\mathbb{R}^d$ denotes the weights of the network at the current iteration $t$, and the expectation is with respect to the true distribution of the samples $(X,Y)$. Assume there are $n$ distributed nodes and each node $i$ for $i=1,\dots,n$ computes the (stochastic) gradient of the loss function with respect to  a small batch of i.i.d. samples $\{(X_{j}^{(i)}, Y_{j}^{(i)})\}_{j=1}^{B}$ available at this node,
$$
g_i^t=\frac{1}{B}\sum_{j=1}^B \nabla \ell (\omega_t;(X_{j}^{(i)},Y_{j}^{(i)})).
$$
Note that when disjoint subsets of the dataset are assigned to different nodes, $\{(X_{j}^{(i)}, Y_{j}^{(i)})\}_{j=1}^{B}$ can be modeled as independent and identically distributed for different $i$. Hence, the local gradients $g_1^t, g_2^t,\dots, g_n^t\,\in\,\mathbb{R}^d$ are generated independently from the same (unknown) distribution  and have mean equal to $g^t$, the true gradient with respect to the population risk. \footnote{The same model can be extended to the case where nodes perform multiple steps of stochastic gradient descent on their local dataset such as in federated learning \cite{fedreview}, in which case $g_i^t$ is the resultant model update generated by node $i$.} To model the communication bottleneck, assume each node has $k$ bits to communicate its local gradient vector $g_i^t$ to the master node. The goal of the master node is to generate an estimate $\hat{g}^t$ of the true gradient $g^t$ under squared $\ell^2$ risk as per \eqref{minmax} from the  $nk$-bit transcript $M$ it obtains at the end of this communication round. The $g^t$ can be regarded as the parameter of the underlying distribution that we wish to estimate. In order to complete the model description,  we need to specify the statistical model $P_\theta$, with $\theta=g^t$, according to which the samples $g_1^t, g_2^t,\dots, g_n^t$ are generated and the set $\Theta\subseteq\mathbb{R}^d$ in which the parameter lies.

\begin{figure}
\centering
\begin{tikzpicture}
\node at (2, 1.4) {$g^t=\mathbb{E}[\nabla \ell (\omega;(X,Y))]$}; 
\draw [->] (1.8, 1.2) -- (0.2, 0.2); 
\draw [->] (1.9, 1.2) -- (1.1, 0.2); 
\draw [->] (2.1, 1.2) -- (2.9, 0.2); 
\draw [->] (2.2, 1.2) -- (3.8, 0.2); 
\draw (0,0) circle (0.2cm); \node [below] at (0,-0.2) {$\tilde{g}_1^t$}; 
\draw (1,0) circle (0.2cm); \node [below] at (1,-0.2) {$\tilde{g}_2^t$}; 
\node at (2,0) {$\cdots$}; 
\draw (3,0) circle (0.2cm); \node [below] at (3,-0.2) {$\tilde{g}_{n-1}^{t}$}; 
\draw (4,0) circle (0.2cm); \node [below] at (4,-0.2) {$\tilde{g}_{n}^{t}$}; 
\draw [->] (0, -0.7) -- (0, -1.4); \draw [->] (1, -0.7) -- (1, -1.4); 
\draw [->] (3, -0.7) -- (3, -1.4); \draw [->] (4, -0.7) -- (4, -1.4);
\draw (-0.3,-2.5) rectangle (4.3,-1.5);  % \node at (2,-3) {transcript $Y$}; 
\node at (2,-2) {centralized processor}; 
\draw [->] (4.3,-2) -- (5, -2); \node [right] at (5,-2) {$\hat{g}^t$}; 
%\draw [->] (2,-2.5) -- (2, -3); \node [below] at (2,-3) {$\hat{g}^t$}; 
\node [left] at (0, -1) {$k$ bits}; \node [right] at (4,-1) {$k$ bits}; 
\end{tikzpicture} 
\caption{Statistical estimation model for distributed training.}
\label{fig:fig1}
\end{figure} 

\subsection{Statistical Models}

The distributed parameter estimation problem in \eqref{minmax} has been studied for specific classes of statistical models $P_\theta$ in the literature. One canonical model that has been of significant interest in the literature is the Gaussian location model $P_\theta=\mathcal{N}(\theta,\sigma^2I_d)$ with $\Theta=\mathbb{R}^d$ which is studied in \cite{duchi,garg,braverman,yanjun}. Adopting this Gaussian model for the gradient aggregation problem would correspond to modeling the local gradients $g_i^t$ computed at each node as i.i.d. observations of the true gradient vector $g_t$ under spherically-symmetric additive Gaussian noise. However, this leads to dense observation vectors $g_i^t$, while the distribution of the local gradients is often skewed and sparse like in experiments, i.e. often relatively few entries of $g_i^t$ have large magnitudes and many entries have magnitudes close to zero. 

A sparse variation of the Gaussian mean estimation problem has been studied in \cite{garg,braverman, yanjun}, where $\Theta= \{\theta\in \mathbb{R}^d:\|\theta\|_0\le s\le d\}$. Adopting this statistical model for the gradient aggregation problem would correspond to modeling the true gradient vector $g_t$ as sparse, with only $s$ non-zero components, while the local gradients $g_i^t$ computed at each node would still correspond to i.i.d. observations of the true gradient vector $g_t$ under additive Gaussian noise. Even though the true gradient vector $g_t$ is assumed to be sparse, qualitatively this model behaves similarly to the original Gaussian model. In particular the number of bits $k$ needed to achieve the centralized estimation performance (with no communication constraints) scales linearly with the ambient dimension $d$ as in the original Gaussian model, i.e. it is not impacted by the sparsity $s$. Similarly the optimal communication scheme independently quantizes each gradient component as in the case of the dense Gaussian model.

In this work, we instead propose to focus on the following sparse Bernoulli model. Suppose each node $i$ has a sample \begin{equation}\label{eq:model} X_i \sim \prod_{j=1}^d\text{Bern}(\theta_j)\end{equation} with $$\Theta = \left\{ \theta\in[0,1]^d \, : \, \sum_{j=1}^d \theta_j \leq s \right\} \; .$$ This model imposes a soft sparsity constraint on the parameter vector $\theta$; when $s\ll d$ not all entries of $\theta$ can be large, i.e. close to `1'. The observation vectors $X_i$ are highly skewed with entries either equal to `1' or `0'. Note also that the parameter vector $\theta$ corresponds to the mean of the observation vectors $X_i$. We adopt this model for the gradient aggregation problem with the understanding that $\theta=|g_t|$ and the `0' values from the Bernoulli random variables model entries of $g_i^t$ with small magnitudes, while the `1' values model entries with large magnitudes. Note that a large value for a given component of $\theta=|g_t|$ makes it more likely to observe `1', i.e. a large magnitude entry in the corresponding location of the stochastic gradient vectors $g_i^t$ for $i=1,\dots,n$. However, it does not exclude the possibility of observing a `0' i.e. a small magnitude entry, in the same location.

While this is a highly simplified model for real stochastic gradient vectors, it allows us to focus our attention on the impact of a highly skewed distribution for the magnitudes of the gradients. This model and our main results in the next section can be easily extended to more accurately reflect the distribution of the stochastic gradients, and doing so does not change the optimal encoding or estimation schemes. In particular, we could consider the following refinements:
\begin{itemize}
\item[(i)]{\bf Signed values:} The mean parameters $\theta_j$ could be in $[-1,1]$ subject to $\sum_{j=1}^d |\theta_j| \leq s$, so that  $\theta_j$'s can be positive or negative, with the $j$th component of the $X_i$ now being $\mathsf{Sign}(\theta_j)\mathsf{Bern}(|\theta_j|)$.
\item[(ii)]{\bf Scaling:} The Bernoulli random variables could be scaled by any $M>0$ with the goal of estimating the scaled Bernoulli parameters $M\theta$.
\item[(iii)]{\bf Continuous Perturbations:} We could add a vector of continuous independent zero-mean random variables $Z_i$ to each $X_i$,  where $X_i$ is distributed according to \eqref{eq:model} and each component of $Z_i$ is supported in $[-\frac{1}{2},\frac{1}{2}]$. As a result, each component of the resultant $Y_i=Z_i+X_i$ will now take continuous values.
\end{itemize}
With none of these refinements changing the fundamental encoding and estimation schemes, we find that the simple sparse Bernoulli model captures the issues that are central to our distributed estimation problem. Note that by including just the sign and scaling changes, the resulting model also makes a good representation of coarsely quantized stochastic gradients such as with ternary quantization.

%\begin{thm}[Sparse Gaussian location model]\label{thm.sparse}
	%Let $P_{\theta}=\mathcal{N}(\theta,\sigma^2I_d)$ with $\Theta= \{\theta\in \mathbb{R}^d:\|\theta_0\|\le s\}$. For $k\ge \log d$ and $n\ge \frac{sd\log(d/s)}{\min(k,d)}$, we have
	%\begin{align}
	%\inf_{\left(\Pi\in\Pi_{\mathsf{BB}},\hat{\theta}\right)}\;\sup_{\theta\in\Theta} \mathbb{E}_{\theta}\|\hat{\theta}-\theta\|_2^2 =\Theta \left(\max\left(\frac{sd\sigma^2\log(d/s)}{nk}, \frac{s\sigma^2\log(d/s)}{n}\right)\right). \label{eq:sparseG}
	%\end{align}
	%\end{thm}
%
%The bound in the theorem can be achieved with a simple independent communication protocol to within a logarithmic gap. For $k\leq d$, we partition the $d$ dimensions into $d/(k/c)$ segments each of size $k/c$ for $c=\Theta(\log n)$. Each node is assigned a segment, hence each segment is assigned to $nk/dc$ different nodes. Each node $i$ only communicates the entries of its sample vector $X_i$ in its assigned segment by quantizing each entry into $c$ bits, hence using $c\times k/c$ bits in total. The central node then averages all of the quantized samples it has for each component, and sets any component to zero if it has magnitude less than a constant fraction times $\sigma/\sqrt{n}$ (see \cite{garg}).
%
%This model allows the underlying parameter $\theta$ to have $s\leq d$ non-zero components, where $s=d$ corresponds to the non-sparse case. The samples $X_i$ correspond to observations of $\theta$ under spherically-symmetric i.i.d. Gaussian noise. In the gradient aggregation problem, this would correspond to assuming that the true gradient vector $g_t$ is $s$-sparse and the local gradients $g_i^t$ computed at each node correspond to observations of $g_t$ under independent Gaussian noise. Note that under this model, even if the mean $\theta$ is assumed to be sparse, the sample vectors $X\sim\mathcal{N}(\theta,\sigma^2I_d)$ are dense since noise of constant variance is added to each entry of $\theta$. As a result, in \eqref{eq:sparseG}, the number of bits $k$ (per node) needed to achieve the centralized performance is linear in $d$ regardless of the sparsity level $s$. (The centralized performance is given by the second term in the maximization on the right side of \eqref{eq:sparseG}.) However in experiments, the stochastic gradient vectors $g_i^t$ computed at each node have been observed to be sparse-like: only a small subset of the $d$ dimensions have large magnitudes while most entries have magnitude close to zero.  Experimental results have also shown that the centralized performance can be achieved by using much fewer than $d$ bits per node. In the next section, we propose a model that better captures the statistical characteristics of the gradient vectors. 

%Nevertheless, it is worth noting that the optimal scheme for the sparse Gaussian location model suggests the idea of segmentation for communicating the sample vectors when communication budget is limited: different segments of the gradient vector can be computed by different nodes on their respective local datasets and segments can be aggregated at the central node. We experiment with this strategy in Section~\ref{sec:experiments}.

\subsection{Theoretical Results and Discussion}

%This reflects the fact that the stochastic gradient vectors, which themselves are relatively sparse, may have large entries even in locations where the true gradient vector is small. The Bernoulli model captures the fact that the entries of the stochastic gradient vectors are also sparse like, with some entries having magnitudes much larger than others. This model may also be useful for analyzing stochastic gradient vectors after they have been thresholded, where many entries are set directly to zero, or after a coarse 1-bit quantization where the entries are set directly to zero or one.

We now turn to analyzing the distributed estimation problem under this model.

\begin{thm}[sparse Bernoulli upper bound]\label{thm:sparseBernoulliUB}
For the sparse Bernoulli model \eqref{eq:model} above,
$$\inf_{(\hat\theta,\Pi_i)}\sup_{\theta\in\Theta} \mathbb{E}_\theta\|\hat\theta-\theta\|_2^2 \leq C\frac{s^2\log d}{nk}$$
for $2\log d \leq k \leq s\log d$ and some constant $C$ that is independent of $n,k,d,s$.
\end{thm}

We prove this theorem in Section~\ref{sec:SparseBUB} by describing an explicit independent encoding scheme at each node and a centralized estimator that together achieve at most this error. The scheme is built on the idea of subsampling the non-zero entries in each sample vector and communicating the locations of the subsampled components. With signed values as in (i) above, the scheme is modified to communicate also the sign of each subsampled component. Since this requires only a single bit for each subsampled component it does change the scalings in Theorem~\ref{thm:sparseBernoulliUB}. Similarly, the constant scaling in (ii) also does not impact the scheme and the result of Theorem~\ref{thm:sparseBernoulliUB}. When continuous perturbations are present as in (iii), the scheme is modified to include a pre-processing step where $Y_i$ is quantized to `0' if $|Y_i|\leq 1/2$, and quantized to `1' if $|Y_i|>1/2$. This converts the observations to the original Bernoulli model, on which we apply the idea of random subsampling. This recovers the result in Theorem~\ref{thm:sparseBernoulliUB}. Note that this strategy is different than simply communicating the components of $Y_i$ with largest magnitude or the indexes of these large magnitude components.

We also prove the following lower bound which shows that our proposed scheme is order optimal up to logarithmic factors.

\begin{thm}[Sparse Bernoulli lower bound] \label{thm:sparseBernoulliLB}
For the sparse Bernoulli model \eqref{eq:model} above, if $nk \geq d\log\frac{d}{s}$ and $s\leq\frac{d}{2}$ then
\begin{equation}
\sup_{\theta\in\Theta} \mathbb{E}_\theta\|\hat\theta-\theta\|_2^2 \geq c\max\left\{\frac{s^2\log \frac{d}{s}}{nk},\frac{s}{n}\right\}\label{eq:sparseBerLB}
\end{equation}
for any estimator $\hat{\theta}(M)$, communication strategies $\Pi_i$, and some constant $c$ that is independent of $n,k,d,s$.
\end{thm} 
The proof is given in Section~\ref{sec:pf2}. It builds on a geometric characterization of Fisher information from quantized samples, a framework introduced in \cite{allerton}. The same lower bound applies trivially to extensions (i) and (ii) above, while the extension to (iii) follows simply from the data processing inequality for Fisher information. The two theorems together show that the number of bits $k$ (per node) needed to achieve the centralized performance under the sparse Bernoulli model is of the order of $s\log d$. (The centralized performance is given by the second term in the maximization on the right side of \eqref{eq:sparseBerLB}.) This model is interesting from a statistical estimation perspective; in contrast to the sparse Gaussian location model, this model suggests that the centralized performance can be achieved with much fewer than $d$ bits when the underlying vector is sparse with $s\ll d$.  

\subsection{rTop-$k$ Algorithm}
\label{sec:rtopk}
The main algorithmic idea that emerges from the theoretical analysis of the sparse Bernoulli model is to communicate a random subset of the large magnitude entries of the local gradient vectors. Motivated by this observation, we propose Algorithm \ref{algorithm_rtopk} for encoding and aggregating gradients so as to reduce the overall communication cost.
\begin{algorithm}[h]
{\bf Hyperparameters:} number of components communicated $k$, subsampling ratio $r/k$ \\
{\bf Inputs:} stochastic gradients $g_1^t,\ldots,g_n^t$ \\
{\bf Output:} an estimate $\hat g^t$ of the true gradient $g^t$ \\
\vspace{-.2in}
\begin{algorithmic}
\State {$\hat g^t \gets 0$}
\For{$i=1,\ldots,n$} \State{$\hat g^t \gets \hat g^t + \mathsf{rTopEncode}(g_i^t)$} \EndFor
\State {$\hat g^t \gets \left(\frac{r}{nk}\right)\cdot\hat g^t$} \\
\State $\mathsf{rTopEncode}(g_i^t):$
\State \hspace{.15in} $I \gets$ (indices of the $r$ largest mag. components of $g_i^t)$
\State \hspace{.15in} $I \gets$ (a random subset of $k$ out of the $r$ elements of $I$)
\State \hspace{.15in} $g \gets$ ($g_i^t$ with indices  not in $I$ set to 0)
\State \hspace{.15in} {\bf return} g
%\vspace{.1in}
\end{algorithmic}
\caption{rTop-$k$}
\label{algorithm_rtopk}
\end{algorithm}

This algorithm first chooses the $r$ entries with largest magnitudes of each local gradient vector and then communicates $k$ randomly chosen gradients among these $r$ entries. It can be viewed as a concatenated application of top-$r$ and random-$k$ strategies, both of which appear in the prior literature. However, the concatenated application of these strategies which we call rTop-$k$ is novel and as we detail in the next section, consistently outperforms either strategy applied alone in experiments. Intuitively, top-$r$ sparsification allows to focus only on the most significant entries of the gradient vector and random-$k$ sparsification allows to reduce the bias introduced by top-$r$ sparsification, hence concatenation combines the best of the two approaches. 

Note that using this algorithm, $k$ is the final number of components that must be communicated from each node to the centralized processor. Since the index for each component can be referred to with $\log d$ bits, and the value of each component can be encoded with a constant number of bits of precision, this is also up to logarithmic factors the number of bits needed for communication. For this reason we have used $k$ to refer to both the number of bits allowed in the distributed statistical estimation framework, and the number of gradient components that are communicated in distributed training.

In Algorithm \ref{algorithm_rtopk_memory}, we show how the rTop-$k$ procedure can be used in distributed SGD with gradient accumulation \cite{deepgrad}. This is the algorithm we use for the simulations in the subsequent section. Distributed SGD with gradient accumulation and compression of the gradients via a ``$k$-contraction'' or ``compression operator'' has been analyzed in \cite{Stichetal} and \cite{Qsparse-local-SGD}, respectively. In these works they show for such operators (Definition 2.1 in \cite{Stichetal} and Definition 3 in \cite{Qsparse-local-SGD}), the SGD converges in the strongly convex \cite{Stichetal} and smooth but non-convex \cite{Qsparse-local-SGD} cases, and they also give upper bounds on the convergence rate. It is straightforward to show that rTop-$k$ satisfies these contraction/compression properties, and so the convergence of Algorithm \ref{algorithm_rtopk_memory} is guaranteed in these same cases by these same results. These results differ somewhat from the standard proofs of SGD convergence in that the gradient estimates can be unbiased, as is the case for rTop-$k$, however this does not affect the convergence of the algorithm.

\begin{algorithm}[!h]
{\bf Hyperparameters:} number of components communicated $k$, subsampling ratio $r/k$, learning rate $\eta$, minibatch size $B$ \\
%{\bf Inputs:} stochastic gradients $g_1^t,\ldots,g_n^t$ \\
{\bf Inputs:} training data $(X^{(i)}, Y^{(i)})$ \\
%{\bf Output:} an estimate $\hat g^t$ of the true gradient $g^t$ \\
{\bf Output:} weights $\omega^T$ \\
\vspace{-.2in}
\begin{algorithmic}
\State{Broadcast randomly initialized weights, $\omega^0$, to all nodes.}
\State{$m_i^0 \gets 0$}
\For{$t=0,\ldots,T-1$} \\
\hspace{.15in} \underline{\textbf{On Nodes:}}
%\State{$\hat g^t \gets 0$}
\For{$i=1,\ldots,n$} 
\State{receive $\omega^{t}$ from the centralized processor.}
\State{$g_i^t \gets \frac{1}{B} \sum_{j=1}^B\nabla \ell (\omega_t;(X_j^{(i)}, Y_j^{(i)}))$}
\State{$\hat g_i^t, \ m_i^{t+1} \gets  \mathsf{rTopEncode}(g_i^t, \ m_i^t)$}
\State{send $\hat g_i^t$ to the centralized processor.} \EndFor \\
\hspace{.15in} \underline{\textbf{On Centralized Processor:}}
\State{receive $\hat g_i^t$s from $n$ nodes.}
\State{$\hat g^t \gets \left(\frac{r}{nk}\right)\cdot\sum_{i=1}^n \hat g_i^t$}  
\State {$\omega^{t+1} \gets \omega^{t} + \eta \cdot \hat g^t$} 
\State{broadcast $\omega^{t+1}$ to all nodes.}
\EndFor \\
\State $\mathsf{rTopEncode}(g_i^t, \ m_i^t):$
\State \hspace{.15in} $g_i^t \gets g_i^t+ m_i^t$
\State \hspace{.15in} $I \gets$ (indices of the $r$ largest mag. components of $g_i^t)$
\State \hspace{.15in} $I \gets$ (a random subset of $k$ out of the $r$ elements of $I$)
\State \hspace{.15in} $\hat g_i^t \gets$ ($g_i^t$ with indices  not in $I$ set to 0)
\State \hspace{.15in} $m_i^{t+1} \gets$ $g_i^t-\hat g_i^t$
\State \hspace{.15in} {\bf return} $\hat g_i^t$, $m_i^{t+1}$
%\vspace{.1in}
\end{algorithmic}
\caption{SGD with rTop-$k$ and Gradient Accumulation}
\label{algorithm_rtopk_memory}
\end{algorithm}


